ChatGraph: Chat with Your Graphs

Graph analysis is fundamental in real-world applications. Traditional approaches rely on SPARQL-like languages or clicking-and-dragging interfaces to interact with graph data. However, these methods either require users to possess high programming skills or support only a limited range of graph analysis functionalities. To address the limitations, we propose a large language model (LLM)-based framework called ChatGraph. With ChatGraph, users can interact with graphs through natural language, making it easier to use and more flexible than traditional approaches. The core of ChatGraph lies in generating chains of graph analysis APIs based on the understanding of the texts and graphs inputted in the user prompts. To achieve this, ChatGraph consists of three main modules: an API retrieval module that searches for relevant APIs, a graph-aware LLM module that enables the LLM to comprehend graphs, and an API chain-oriented finetuning module that guides the LLM in generating API chains.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> sec-back.tex <==
\section{ChatGraph Overview}

A graph $G$ is a tuple $(V,E)$, where $V$ is the set of nodes and $E$ is the set of edges. A node $u$ may have a label $l(u)$. A graph database $D$ is a set of graphs $D=\{G_1,G_2, ..., G_n\}$. 


\subsection{System Overview}

The system is composed of four modules: the graph-aware LLM module, API chain learning, and the approximate nearest neighbor search (ANNS) module. The user inputs a prompt text and a graph $Q$. The LLM module embeds the prompt text of the user and the description text of a graph processing tool to vectors $h_p$ and $h_t$, respectively. The graph embedding module embeds the graph input by the user to a vector $h_Q$.
The ANNS module computes the vector $\bar{h}$ among a set of vectors that is the closest to a given vector. The plugin module invokes the graph processing tool corresponding to $\bar{h}$ to process $Q$.

\vspace{-2ex}
\begin{figure}[thbp] 
\centering
\includegraphics[width=9cm]{figures/archV2}
\caption{System overview}\label{fig:overview}
\vspace{-2ex}
\end{figure}



\subsection{Approximate Nearest Neighbor Search}

\begin{definition}
Given a set $S$ of data vectors, a query vector $h$, and a parameter $\epsilon$, the approximate nearest neighbor search returns a vector $h'$ in $S$ such that $d(h',h)<(1+\epsilon)d(h^*, h)$, where $d$ is the distance function between two vectors and $h^*$ denotes the exact nearest neighbor of $h$ in $S$.
\end{definition}

Recent works \cite{ISsurvey, annsExpt, benchmarkIS20, CompSurveyPGVLDB21} show that the proximity graph (PG) index outperform other indexes on large scale ANNS applications. A PG of $S$ is a graph $\cal G$, where each vertex is a vector in $S$ and two vertices have an edge if the two vectors satisfy some proximity property.




$\tau$-MG \cite{tMG} is the state-of-the-art PG, which has the smallest search time complexity among all existing PGs. The core of $\tau$-MG lies at the edge occlusion rule.

\begin{definition}
(Edge occlusion rule \cite{tMG})
\end{definition}










==> sec-intro.tex <==

\section{Introduction}


Graphs have been widely used to model unstructured data in a lot of real-world applications such as chemi-informatics, bioinformatics, and computer vision, etc. Traditional approaches to interact with graph databases includes the SQL-like language (e.g., SPARQL \cite{} and GraphQL \cite{GQL}) and the clicking-and-dragging interface ({\it e.g.}, GBLENDER \cite{GBLENDER} and CATAPULT \cite{CATAPULT}). However, the former approaches require the users having high programming skills to accurately express their needs which may not be realistic for the domain experts. The latter approaches currently only support a limited types of graph processing functionalities and need great efforts to be extended.

Recently, large language model (LLM)-based frameworks ({\it e.g.}, ChatGPT \cite{}, LongChain \cite{},  Semantic Kernel \cite{}, and Gorilla \cite{}) have become a new trend for data interaction and have attracted a lot of research interests. The third-party data processing tools can be integrated in the LLM-based frameworks. The user specifies her needs using natural language. The LLM recognizes the intent of the user and invokes an appropriate chain of tools. The data interaction using the LLM-based frameworks becomes significantly more easy-to-use and flexible than using the traditional approaches. However, graph data analysis has not been supported by existing LLM-based frameworks.

To address the limitation, this demonstration implements a novel system to interact with graph data, which follows the LLM-based framework. The main idea is embedding the description of each graph processing tool into a vector in the $m$-dimensional Euclidean space $E^m$. When the user specifies her needs by a text, the text is also embedded into a vector in $E^m$. The tool whose vector having the smallest distance with the vector of the user's text is invoked for graph processing.


The main contributions of this work are listed as follows.

\begin{itemize}
\item We design and implement ChatGraph
\item We demonstrate how our ChatGraph works through three demo scenarios on a real-world dataset.
\end{itemize}
